On the Generalization of Models Trained with SGD: Information-Theoretic Bounds and Implications

This paper follows up on a recent work of Neu et al. (2021) and presents some new information-theoretic upper bounds for the generalization error of machine learning models, such as neural networks, trained with SGD. We apply these bounds to analyzing the generalization behaviour of linear and two-layer ReLU networks. Experimental study of these bounds provide some insights on the SGD training of neural networks. They also point to a new and simple regularization scheme which we show performs comparably to the current state of the art.

==> Extension.tex <==
\section{Conclusion and Outlook}
\label{sec:extension}

This paper presents new generalization bounds for models, such as neural networks, trained with SGD, improving upon the results of \cite{neu2021information}. Our bounds naturally point to new and effective regularization schemes. At the same time, they
 reveal interesting phenomena in the SGD training of neural networks.  While these phenomena deserve further investigation in their own right, we here suggest another direction for improving the bounds, namely, via the use of strong data-processing inequalities (DPI) \citep{polyanskiy2015dissipation,polyanskiy2017strong,raginsky2016strong}.
 %(noting that the standard DPI is in fact needed for establishing Theorem \ref{thm:sgd-bound-random}). 

%\paragraph{Strong data-processing inequality and time-decaying factor.} Some researches find that there exists a time-decaying factor in the trajectory term for the SGLD algorithm \cite{mou2018generalization,wang2021learning}. Notably, the strong data-processing inequality (SDPI) used in \cite{wang2021learning} can also be applied here.


% For a Markov chain $U \rightarrow X \rightarrow
% Y$, the well-known data-processing inequality \cite{cover2012elements} states that $I(U; Y ) \leq I(U; X)$. It turns out that this inequality can often be tightened in the form of 
% \begin{equation}
% \label{eq:SDPI_generic}
%     I(U; Y ) \leq \eta I(U; X)
% \end{equation}
% for some $\eta<1$. Such an inequality is referred to as a strong data-processing inequality (SDPI). Note the coefficient $\eta$ fundamentally depends on the contraction property of the stochastic kernel $P_{Y|X}$, characterizing the extent by which the kernel brings two different distributions $P_X$ and $P_{X'}$ closer after the stochastic mapping. As the reader may refer to \cite{polyanskiy2015dissipation, polyanskiy2017strong,raginsky2016strong} for a full exposition of this subject, 
% here for self-containedness, we here make an modest revision of the settings in \cite{polyanskiy2015dissipation, polyanskiy2017strong,raginsky2016strong} and develop slightly finer results concerning the contraction properties of $P_{Y|X}$. Specifically, the contraction coefficient $\eta$ in our setting will not only depend on the kernel $P_{Y|X}$, it will also depend on the ``effective input space'' which the kernel acts upon.  

For any Markov chain $U\rightarrow X \rightarrow Y$, we will denote by ${\cal U}$, ${\cal X}$, and ${\cal Y}$ the spaces in which $U$, $X$, $Y$ take values, respectively. For any distribution $P$ on ${\cal X}$, we will use $P_{Y|X} \circ P$ to denote the distribution on ${\cal Y}$ induced by the push-forward of the distribution $P$ by $P_{Y|X}$, namely, for any $y\in {\cal Y}$,
$
\left(P_{Y|X} \circ P \right)(y) \triangleq 
\int P_{Y|X}(y|x)P(x) dx.
$
Let  ${\cal S}(U)$ be the support of  $P_U$ and ${\cal H}(U, P_{X|U})$ be the convex hull of $\{P_{X|U=u}: u\in {\cal S}(U)\}$.
%, namely, ${\cal H}(U, P_{X|U})$ contains all distributions on ${\cal X}$ which can be expressed as $P_{X|U}\circ P$ for some distribution $P$ on ${\cal U}$ whose support is a subset (not necessarily proper) of ${\cal S}(U)$.  It is apparent that $P_X \in {\cal H}(U, P_{X|U})$. 
%$Given the Markov chain, $U \rightarrow X \rightarrow Y$, we now define the contraction coefficient $\eta$ as
Define
% \begin{equation}
% \label{eq:eta}
\[
    \eta(U\rightarrow X \rightarrow Y) \triangleq \sup_{P, Q \in {\cal H}(U, P_{X|U})} \frac{\mathrm{D_{KL}}(P_{Y|X}\circ P || 
    P_{Y|X}\circ Q)
    }{\mathrm{D_{KL}}(P || Q)}.
\]
%\end{equation}
% where ${\rm KL}$ denotes the KL divergence. We note that this definition of the contraction coefficient differs from the standard definition
% \cite{polyanskiy2015dissipation, polyanskiy2017strong,raginsky2016strong} in that the supremization in the latter is over all $P, Q$ which are distributions on ${\cal X}$, making the contraction coefficient only depends on $P_{Y|X}$. In our definition (\ref{eq:eta}), the coefficient $\eta$ also depends on the ``effective input space'' of the kernel, namely,  ${\cal H}(U, P_{X|U})$. 

% Some standard results concerning the contraction coefficient can be easily extended to this revised definition of $\eta$ in (\ref{eq:eta}), which we state below.

\begin{lem}
For any Markov chain $U\rightarrow  X \rightarrow Y$, 
  $  I(U; Y ) \leq \eta (U\rightarrow X \rightarrow Y) I(U; X).$
% \label{lem:SDPI}
\end{lem}
Here $\eta (U\rightarrow X \rightarrow Y)$ serves as the ``contraction coefficient'' for the stochastic kernel $P_{Y|X}$, characterizing the greatest extent by which the kernel may bring closer any two distributions on ${\cal S}(U)$ in its output space. It is easy to see that  
$\eta (U\rightarrow X \rightarrow Y)\le 1$, giving rise to a stronger DPI.

%We note that the SDPI (\ref{eq:SDPI}) follows easily from the definition of mutual information and that of $\eta$. The inequality (\ref{eq:eta-bound}) is an adaptation, to this context, of the result that the contraction coefficient is upper bounded by the \emph{Dobrushin’s coefficient} of the kernel $P_{Y|X}$ \cite{dobrushin1956central}.


%In this section, we will prove Theorem \ref{thm:sgd-bound-extention} that is a stronger version of Theorem \ref{thm:sgd-bound-random}. To prove Theorem \ref{thm:sgd-bound-random}, we only need to let the contraction coefficient $\eta$ be $1$, meaning using a weak version of data-processing inequality.

%We first apply the SDPI in Lemma \ref{lem:SDPI} to auxiliary weight process and the SGD weight process. 

Denote
%\begin{equation}
    % G_t \triangleq -\lambda_t g(W_{t-1}, B_t),  ~{\rm and} ~
$V_t \triangleq \widetilde{W}_{t-1} + G_t.$
%\end{equation}
%Thus $V_t$ and $\widetilde{W}_t$ differ only by the noise $N_t$, or $\widetilde{W}_{t} = V_t + N_t$. 
% \begin{figure}[ht]
% 	\begin{center}
% 		\scalebox{0.6}{
% 			\input{markovchainfig}
% 			}
% 	\end{center}
% 	 \caption{The relationship between $Z_i$, $\widetilde{W}_t$'s
% $V_t$'s, and $G_t$'s}
% 	 \label{fig:markovprocess_for_zi}
% \end{figure}
%Consider a fixed example $Z_i$ in the training set $S$. Let ${\cal T}_i$ denote the of all batch indices $t$ for which $B_t$ contains $Z_i$.  We will assume that ${\cal T}_i$ contains $K$ indices and consider ${\cal T}_i$ as $\{t_1, t_2, \ldots, t_K\}$. The relationship between $Z_i$, $\widetilde{W}_t$'s, $V_t$'s, and $G_t$'s are shown in Figure \ref{fig:markovprocess_for_zi}. 
It can be verified that $Z_i \rightarrow V_t 
\rightarrow \widetilde{W}_t$ form a Markov chain.
%\footnote{Note that even for $t<t_1$, in which $Z_i$ and $V_t$ are independent, the Markov chain still holds, although it degenerates.}. 
Denote $
\eta_{i, t} \triangleq \eta (Z_i \rightarrow V_t 
\rightarrow \widetilde{W}_t)$,
and $\Gamma_i^t= \{t+1,t+2,\dots,T\}\setminus \mathcal{T}_i$. Theorem \ref{thm:sgd-bound-random} can be improved to:
\begin{thm}
The expected generalization error of SGD is bounded by
\begin{align*}
|\mathrm{gen}(\mu,P_{W_T|S})|\leq&
\frac{2R}{nb}\sum_{i=1}^n\sqrt{\sum_{t\in\mathcal{T}_i}\frac{\lambda_t^2 }{\sigma_t^2}\ex{}{\mathbb{V}(W_{t-1})}\cdot\prod_{\substack{\tau\in\Gamma_i^t}} \eta_{i,\tau}}+|\mathbb{E}\left[\gamma(W_T,S)-\gamma(W_T,S')\right]|.
\end{align*}
\label{thm:sgd-bound-extention}
%where 
%$0<\eta_{i,\tau}, \leq 1$
%$\Gamma_i^t= \{t+1,t+2,\dots,T\}\setminus \mathcal{T}_i$.
%$\mathcal{T}_i$ is the set of indices of iterations that use the sample $Z_i$ given a specific sample path.
\end{thm}

%The time-decaying factor may be inevitable in a generalization bound of SGD since it could characterize the impact of different phase of training on the generalization . Unfortunately, we are unable to estimate a meaningful $\eta_{i,\tau}$ in practice, and using Dobrushin's coefficient to upper bound it is too pessimistic.

%\section{Concluding Remarks}Assume the hypothesis space $\mathcal{W}$ is compact with diameter $\gamma$, and $||\nabla_w\hat{\ell}(w,z)||_2\leq L$ for any $w$ and $z$. The loss $\ell(w, Z)$ is $R$-subgaussian for any $w \in \mathcal{W}$.  For each epoch, all the training data points are sampled without replacement and are divided into $m$ disjoint mini-batches with batch size $b$ (i.e., $n=bm$ and $T=mK$).

 It remains to characterize the contraction coefficient $\eta_{i, \tau}$ in a computable form. Simply bounding it via the Dobrushin's coefficient \citep{dobrushin1956central}, as suggested in \cite{wang2021learning} for analyzing SGLD, is unlikely to make the bound in this theorem significantly tighter than that in Theorem \ref{thm:sgd-bound-random}. 
